TCAB: A Large-Scale Text Classification Attack Benchmark

We introduce the Text Classification Attack Benchmark (TCAB), a dataset for analyzing, understanding, detecting, and labeling adversarial attacks against text classifiers. TCAB includes 1.5 million attack instances, generated by twelve adversarial attacks targeting three classifiers trained on six source datasets for sentiment analysis and abuse detection in English. Unlike standard text classification, text attacks must be understood in the context of the target classifier that is being attacked, and thus features of the target classifier are important as well. TCAB includes all attack instances that are successful in flipping the predicted label; a subset of the attacks are also labeled by human annotators to determine how frequently the primary semantics are preserved. The process of generating attacks is automated, so that TCAB can easily be extended to incorporate new text attacks and better classifiers as they are developed. In addition to the primary tasks of detecting and labeling attacks, TCAB can also be used for attack localization, attack target labeling, and attack characterization. TCAB code and dataset are available at https://react-nlp.github.io/tcab/.

==> TCAB_ A Large-Scale Adversarial Text Attack Benchmark Dataset/misc-text.tex <==

% [DANIEL] Text deleted from 3.6 Human Evaluation
% We requested evaluations from five different workers on every perturbed example for an averaged score to alleviate the extreme cases.
% Workers were asked to share additional comments when they could not decide on the emotion of a text.

% One HIT represents a perturbed sample. We paid $0.1$ USD for each HIT for all datasets except IMDB. On average, we collected $5$ unique evaluation results for every example with a total of $30$ examples per attack per target model and per dataset. IMDB examples have much longer texts, therefore we paid $0.2$ USD for a HIT, and we collected evaluations for $15$ examples/attack/target model/dataset accordingly.

%We requested evaluations from five different workers for each perturbed example to alleviate outliers and obtain more robust results. 

==> TCAB_ A Large-Scale Adversarial Text Attack Benchmark Dataset/thoughts.tex <==
\daniel{
CLAIM 1: There are important tasks to be done and evaluated 

Specifically: distinguishing attacks from clean text, labeling attack algorithms based on their text, labeling attack targets (distinguishing which model was attacked). 

CLAIM 2: Those tasks are well-supported by this dataset.

CLAIM 2A: We have chosen appropriate attacks for these tasks. 

CLAIM 2B: We have chosen appropriate source datasets for these tasks.

CLAIM 3: Success on this dataset means something in terms of solving an actual problem that people care about (or should care about).

CLAIM 4: Other datasets do not fill this niche.
SUPPORT: List the closest alternatives and why they don't do this.
}


==> misc-text.tex <==

% [DANIEL] Text deleted from 3.6 Human Evaluation
% We requested evaluations from five different workers on every perturbed example for an averaged score to alleviate the extreme cases.
% Workers were asked to share additional comments when they could not decide on the emotion of a text.

% One HIT represents a perturbed sample. We paid $0.1$ USD for each HIT for all datasets except IMDB. On average, we collected $5$ unique evaluation results for every example with a total of $30$ examples per attack per target model and per dataset. IMDB examples have much longer texts, therefore we paid $0.2$ USD for a HIT, and we collected evaluations for $15$ examples/attack/target model/dataset accordingly.

%We requested evaluations from five different workers for each perturbed example to alleviate outliers and obtain more robust results. 

==> thoughts.tex <==
\daniel{
CLAIM 1: There are important tasks to be done and evaluated 

Specifically: distinguishing attacks from clean text, labeling attack algorithms based on their text, labeling attack targets (distinguishing which model was attacked). 

CLAIM 2: Those tasks are well-supported by this dataset.

CLAIM 2A: We have chosen appropriate attacks for these tasks. 

CLAIM 2B: We have chosen appropriate source datasets for these tasks.

CLAIM 3: Success on this dataset means something in terms of solving an actual problem that people care about (or should care about).

CLAIM 4: Other datasets do not fill this niche.
SUPPORT: List the closest alternatives and why they don't do this.
}

